Optimal Strategies to Steer and Control Water Waves

In this paper, we propose a novel approach for controlling surface water waves and their interaction with floating bodies. We consider a floating target rigid body surrounded by a control region where we design three control strategies of increasing complexity: an active strategy based on controlling the pressure at the air-water interface and two passive strategies where an additional controlled floating device is designed. We model such device both as a membrane and as a thin plate and study the effect of this modelling choice on the performance of the overall controlled system. We frame this problem as an optimal control problem where the underlying state dynamics is represented by a system of coupled partial differential equations describing the interaction between the surface water waves and the floating target body in the frequency domain. An additional intermediate coupling is then added when considering the control floating device. The optimal control problem then aims at minimizing a cost functional which weights the unwanted motions of the floating body. A system of first-order necessary optimality conditions is derived and numerically solved using the finite element method. Numerical simulations then show the efficacy of this method in reducing hydrodynamic loads on floating objects.

==> Sections/OLD_0_Abstract.tex <==
Offshore floating wind turbines are of increasing interest in the last decade since the high quality offshore wind guarantees a good reliability in energy production. However, their application in such an adverse environment requires a lot of effort from many research fields. In particular, the detrimental effect on the turbines structural fatigue life caused by vibrations has stimulated the development of many control methods, either active or passive, for limiting unwanted motions. Differently from the usual TMD-based techniques, in this paper we propose a novel approach that limits the turbine motion by acting on the surrounding water flow such that the hydrodynamic forces interacting with the submersed structure have a reduced effect. With this aim, we recast the minimization of turbine detrimental motions as an Optimal Control Problem constrained by a system of coupled Partial Differential Equations. We explore three main strategies: an active one is based on controlling the pressure on the water surface surrounding the turbine; conversely, two passive strategies are developed by designing two floating devices having the dynamics of a membrane and of a thin plate, respectively.

==> Sections/OLD_1_Introduction.tex <==
% Scaletta:
% - problema: energy supply -> offshore -> turbine oscillano per le onde
% - Introduzione onda
% - devices per ww control
% - ambito cloak, soprattutto tramite transformation -> pro tutte freq, limiti sulla forma, cit Davide -> IRREALIZZABILE perché anisotropo 
% - tramite optimization forma generica, considero anche la forma sommersa e la dinamica del body che, siccome non è un cloak perfetto, serve. Ma narrow band (però va bene narrow: ci servono poche frq) -> cit Seba
% - che però sono limitate etc. (tipo la storia del controllo tramite massa >0 galleggiante) One can think of placing many floating masses for controlling, but ...
% - 3 tipi di controllo: a, b e c basati rispettivamente su pressione, modello ice 1, modello ice 2
% 
% DEVO sottolineare le 



% Parlare di ww control, varie possibilità e limiti p.e. del controlllo del fondale
% dire di tecniche cloak, che però sono limitate etc. (tipo la storia del controllo tramite massa >0 galleggiante), e poi sono limitate rispetto alla forma che cloakkano -> cit cloak ellittico


Nowadays, the demand for renewable sources of energy is of growing importance. Among all the emerging strategies, installing offshore turbines for harnessing the wind energy is undoubtedly a clever solution because of the presence of high quality wind; however, to produce energy in marine environments represents a challenge from many engineering points of view. Indeed, it requires to face problems such as energy transport, maintenance and building issues; moreover, hostile natural phenomena, e.g.\ corrosion and biofouling, compromise the turbine's structure integrity \cite{adedipe2016review} but one of the most bothering issues come from cyclic wind and water loads. On one hand, the interaction with air flow is essential to produce energy, on the other hand, the motion generated by water waves has a detrimental effect only. 

As all oscillating phenomena, water waves have a characteristic period that depends on the main restoring force influencing the motion; in particular, their dynamics in the engineering scales considered is mainly governed by gravity and the characteristic time period ranges from \SIrange{1}{25}{\second} \cite{mei2005theory}.
The resulting waves are known as wind waves, swells or, in case of even larger time periods, tsunamis. In particular, swells are steady-state full developed water waves generated by distant storms, and are characterized by narrowband spectra \cite{hasselmann1973measurements}.

During their service life, wind turbines are constantly subjected to cyclic loads coming from the environment and, since their structures are typically built with light-weight and high-strength materials, that are low damped, vibration phenomena are critical for fatigue life; moreover, excessive oscillations can compromise the energy production too. As a result, many strategies usually based on Tuned Mass Dampers have been investigated for reducing unwanted motions; the reader is referred to \cite{zuo2020state} for a recent review on the topic.

Inspired by the cloaking theory originally developed by \cite{leonhardt2006optical,pendry2006controlling} for electromagnetic waves, over the last two decades many effort has been spent in diverse research fields, e.g.\ acoustics \cite{cummer2007one}, elastodynamics \cite{norris2011elastic}, heat conduction \cite{schittny2013experiments}, and water waves too.
Farhat et Al.\ \cite{farhat2008broadband} first applied the transformation theory to water waves, and proposed a structure made of many masses piercing the fluid that, coupled with a proper sea bed shape, allows to limit water actions on a submersed structure; later, a similar approach was proposed by \cite{porter2014cloaking}. However, these methods are of difficult implementation for the case in exam in this work because floating devices are mostly installed in deep sea zones and the sea bed shape is of little influence for wave propagation.\\
A particular device was theorized by \cite{zareei2016cloaking}, probably inspired by the models developed since the middle of the last century about the dynamics of floating ice in oceans \cite{keller1953water,fox1990reflection}. They designed a thin floating plate that surrounds a circular infinite cylinder in constant depth environment; the properties of such a plate are obtained by applying the conformal mapping method \cite{leonhardt2006optical}. Actually, this solution bases on assumptions that must be released in case of floating objects because the obstacle is considered fixed and must extend till the sea bed; but the most restrictive requirement in that case is that the resulting plate is expected to be anisotropic and inhomogeneous, so of difficult realization. 
% \commenti{Moreover, from \cite{zareei2016cloaking} it is not clear if a perfect cloak, designed for scatter reduction purposes, guarantees that the overall forces on the structure is null or even reduced.}

In this paper, we propose a novel approach that considers the floating body dynamics and its whole interaction with water; also, the exposed technique allows to design devices a step closer to real applications. In particular, we investigate active and passive control strategies that interact on the water surface surrounding a floating body.\\
The turbines motion can be measured by a cost function, so the problem is addressed as an Optimal Control Problem (OCP) constrained by a system of coupled Partial Differential Equations (PDEs) that governs the linearized dynamics. In search of an optimal solution, we derive first order necessary conditions, by applying the formal Lagrange's multiplier method \cite{manzonioptimal}, so a gradient based algorithm allows the numerical solution of some test cases. \\
A remarkable advantage of this approach is that problems of arbitrary geometries can be considered, which is of great importance in real applications. Moreover, similar to \cite{cominelli2022design}, where a method for designing acoustic cloaks by solving PDE-constrained OCPs is proposed, we expect that a narrowband high-performance device will be achieved, and this is a good premise for application involving swells.


In the following, we first review the main assumptions of the model adopted, then in section~\ref{sec:pressure controlled} we propose an active control strategy that modifies the pressure on the air/water interface surrounding the floating turbine.
Although this is hardly an implementable solution as it is presented, the results obtained pave the way for innovative control strategies; indeed, the OCP results in a Linear Quadratic one so fast control techniques can be implemented for real-time applications, also by taking benefit from Model Order Reduction techniques \cite{sinigaglia2022fast}. % uno di Jacopo?
This control strategy probably suites well for floating systems such as Floating Production Storage and Offloading (FPSO), where energy can be spent for active control, but this is hardly the case of floating turbines.

Then, in section~\ref{sec:membrane controlled} and \ref{sec:plate controlled}, we explore two passive strategies that consist in covering a portion of the water surface around the turbine with a floating elastic membrane or a plate, respectively. The two models describing the couple dynamics have been originally proposed for studying the effect of floating ice on water waves \cite{keller1953water,fox1990reflection}, and they now come in handy as constraints for the OCP. In particular, the control is tuned by modifying stiffness and inertia properties of the control surface: by increasing the local stiffness, water waves experiment a speed up, conversely they are slowed down as the inertia increases. Note that thanks to this framework, we can impose membrane and plate to be isotropic, so enhancing the manufacturing.
\commenti{Qui sicuramente mancano cose relative alle sezioni}

% Cose che potrei forse citare
% - controllo tramite profondità, tipo quello a lamelle di spessore infinitesimo che si compportano in modo anisotropo
% - 

% Idee su cose da dire
% - C'è più energia verso la superficie -> usiamola!
% - Mi aspetto che l'azione del vento sia correlata

% Idee di cose da fare
% - Analisi prestazioni cloak per una banda di interesse

